Block Coordinate Descent Methods for Optimization under J-Orthogonality Constraints with Applications

The J-orthogonal matrix, also referred to as the hyperbolic orthogonal matrix, is a class of special orthogonal matrix in hyperbolic space, notable for its advantageous properties. These matrices are integral to optimization under J-orthogonal constraints, which have widespread applications in statistical learning and data science. However, addressing these problems is generally challenging due to their non-convex nature and the computational intensity of the constraints. Currently, algorithms for tackling these challenges are limited. This paper introduces JOBCD, a novel Block Coordinate Descent method designed to address optimizations with J-orthogonality constraints. We explore two specific variants of JOBCD: one based on a Gauss-Seidel strategy (GS-JOBCD), the other on a variance-reduced and Jacobi strategy (VR-J-JOBCD). Notably, leveraging the parallel framework of a Jacobi strategy, VR-J-JOBCD integrates variance reduction techniques to decrease oracle complexity in the minimization of finite-sum functions. For both GS-JOBCD and VR-J-JOBCD, we establish the oracle complexity under mild conditions and strong limit-point convergence results under the Kurdyka-Lojasiewicz inequality. To demonstrate the effectiveness of our method, we conduct experiments on hyperbolic eigenvalue problems, hyperbolic structural probe problems, and the ultrahyperbolic knowledge graph embedding problem. Extensive experiments using both real-world and synthetic data demonstrate that JOBCD consistently outperforms state-of-the-art solutions, by large margins.

==> mybib.tex <==

@inproceedings{Mairal13,
  author    = {Julien Mairal},
  title     = {Optimization with First-Order Surrogate Functions},
  booktitle = {International Conference on Machine Learning (ICML)},
  volume    = {28},
  pages     = {783--791},
  year      = {2013},
}
@article{RazaviyaynHL13,
  author    = {Meisam Razaviyayn and
               Mingyi Hong and
               Zhi{-}Quan Luo},
  title     = {A Unified Convergence Analysis of Block Successive Minimization Methods for Nonsmooth Optimization},
  journal   = {SIAM Journal on Optimization},
  volume    = {23},
  number    = {2},
  pages     = {1126--1153},
  year      = {2013},
}


@article{yuan2023block,
  title={A Block Coordinate Descent Method for Nonsmooth Composite Optimization under Orthogonality Constraints},
  author={Ganzhao Yuan},
  journal={ArXiv},
  year={2023},
  volume={abs/2304.03641},
}
@article{bojanczyk2003solving,
  title={Solving the indefinite least squares problem by hyperbolic QR factorization},
  author={Bojanczyk, Adam and Higham, Nicholas J and Patel, Harikrishna},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={24},
  number={4},
  pages={914--931},
  year={2003},
  publisher={SIAM}
}
@article{fawzi2021faster,
  title={Faster proximal algorithms for matrix optimization using Jacobi-based eigenvalue methods},
  author={Fawzi, Hamza and Goulbourne, Harry},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={11397--11408},
  year={2021}
}
@article{higham2003j,
  title={J-orthogonal matrices: Properties and generation},
  author={Higham, Nicholas J},
  journal={SIAM review},
  volume={45},
  number={3},
  pages={504--519},
  year={2003},
  publisher={SIAM}
}
@article{Gau2018,
	author = {Gao, Bin and Liu, Xin and Chen, Xiaojun and Yuan, Ya-xiang},
	title = {A New First-Order Algorithmic Framework for Optimization Problems with Orthogonality Constraints},
	journal = {SIAM Journal on Optimization},
	volume = {28},
	number = {1},
	pages = {302-332},
	year = {2018},
}

@article{Gau2019,
	author = {Gao, Bin and Liu, Xin and Yuan, Ya-xiang},
	title = {Parallelizable Algorithms for Optimization Problems with Orthogonality Constraints},
	journal = {SIAM Journal on Scientific Computing},
	volume = {41},
	number = {3},
	pages = {A1949-A1983},
	year = {2019},
}

@article{xiao2020class,
	title={A class of smooth exact penalty function methods for optimization problems with orthogonality constraints},
	author={Liu, Wei and Zhang, Yinyu and Yang, Hongqiao and Zhang, Shuzhong},
	journal={Optimization},
	volume={69},
	number={3},
	pages={399--426},
	year={2020},
	publisher={Taylor \& Francis}
}

@article{Stewart2005,
author = {Stewart, Michael and Van Dooren, Paul},
title = {On the Factorization of Hyperbolic and Unitary Transformations into Rotations},
journal = {SIAM Journal on Matrix Analysis and Applications},
volume = {27},
number = {3},
pages = {876-890},
year = {2005},
}

@article{Tabaghi2023PrincipalCA,
  title={Principal Component Analysis in Space Forms},
  author={Puoya Tabaghi and Michael Khanzadeh and Yusu Wang and Sivash Mirarab},
  journal={ArXiv},
  year={2023},
  volume={abs/2301.02750},
  url={https://api.semanticscholar.org/CorpusID:255546578}
}

@InProceedings{HoroPCA,
  title = 	 {HoroPCA: Hyperbolic Dimensionality Reduction via Horospherical Projections},
  author =       {Chami, Ines and Gu, Albert and Nguyen, Dat P and Re, Christopher},
  booktitle = 	 {International Conference on Machine Learning (ICML)},
  pages = 	 {1419--1429},
  year = 	 {2021},
  volume = 	 {139},
}

@article{SLAPNICAR200057,
title = {Relative perturbation theory for hyperbolic eigenvalue problem},
journal = {Linear Algebra and its Applications},
volume = {309},
number = {1},
pages = {57-72},
year = {2000},
author = {Ivan Slapnicar and Ninoslav Truhar},
}


@article{Quaequation,
  title={Quartic equation},
  author={WikiContributors},
  journal={\url{https://en.wikipedia.org/wiki/Quartic_equation}}
}

@article{Wen2012AFM,
  title={A feasible method for optimization with orthogonality constraints},
  author={Zaiwen Wen and Wotao Yin},
  journal={Mathematical Programming},
  year={2012},
  volume={142},
  pages={397 - 434},
  url={https://api.semanticscholar.org/CorpusID:10155814}
}

@inproceedings{xiong2022ultrahyperbolic,
  title={Ultrahyperbolic knowledge graph embeddings},
  author={Xiong, Bo and Zhu, Shichao and Nayyeri, Mojtaba and Xu, Chengjin and Pan, Shirui and Zhou, Chuan and Staab, Steffen},
  booktitle={Proceedings of the 28th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={2130--2139},
  year={2022}
}

@article{law2021ultrahyperbolic,
  title={Ultrahyperbolic neural networks},
  author={Law, Marc},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={22058--22069},
  year={2021}
}

@article{chen2021probing,
  title={Probing BERT in hyperbolic spaces},
  author={Chen, Boli and Fu, Yao and Xu, Guangwei and Xie, Pengjun and Tan, Chuanqi and Chen, Mosha and Jing, Liping},
  journal={ICLR},
  year={2021}
}


@inproceedings{hewitt2019structural,
  author       = {John Hewitt and
                  Christopher D. Manning},
  editor       = {Jill Burstein and
                  Christy Doran and
                  Thamar Solorio},
  title        = {A Structural Probe for Finding Syntax in Word Representations},
  booktitle    = {Proceedings of the 2019 Conference of the North American Chapter of
                  the Association for Computational Linguistics: Human Language Technologies (NAACL-HLT)},
  pages        = {4129--4138},
  year         = {2019},
}

@article{Xiong2021SemiRiemannianGC,
  title={Semi-Riemannian Graph Convolutional Networks},
  author={Bo Xiong and Shichao Zhu and Nico Potyka and Shirui Pan and Chuan Zhou and Steffen Staab},
  journal={ArXiv},
  year={2021},
  volume={abs/2106.03134},
  url={https://api.semanticscholar.org/CorpusID:235358415}
}

@inproceedings{nickel2018learning,
  title={Learning continuous hierarchies in the lorentz model of hyperbolic geometry},
  author={Nickel, Maximillian and Kiela, Douwe},
	booktitle={International Conference on Machine Learning},
  pages={3779--3788},
  year={2018},
  organization={PMLR}
}

@inproceedings{yuan2023fractional,
	title={Coordinate descent methods for fractional minimization},
	author={Yuan, Ganzhao},
	booktitle={International Conference on Machine Learning},
	pages={40488--40518},
	year={2023},
}

@inproceedings{yuan2023smoothing,
	title={Smoothing Proximal Gradient Methods for Nonsmooth Sparsity Constrained Optimization: Optimality Conditions and Global Convergence},
	author={Yuan, Ganzhao},
	booktitle={International Conference on Machine Learning},
	year={2024},
}
@inproceedings{KingmaB14,
  author       = {Diederik P. Kingma and
                  Jimmy Ba},
  editor       = {Yoshua Bengio and
                  Yann LeCun},
  title        = {Adam: {A} Method for Stochastic Optimization},
  booktitle    = {International Conference on Learning Representations (ICLR)},
  year         = {2015},
}
@inproceedings{yuan2020block,
	title={A block decomposition algorithm for sparse optimization},
	author={Yuan, Ganzhao and Shen, Li and Zheng, Wei-Shi},
	booktitle={Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
	pages={275--285},
	year={2020}
}


@article{yu2019numerically,
  title={Numerically accurate hyperbolic embeddings using tiling-based models},
  author={Yu, Tao and De Sa, Christopher M},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@article{chen2021fully,
  title={Fully hyperbolic neural networks},
  author={Chen, Weize and Han, Xu and Lin, Yankai and Zhao, Hexu and Liu, Zhiyuan and Li, Peng and Sun, Maosong and Zhou, Jie},
  journal={arXiv preprint arXiv:2105.14686},
  year={2021}
}

@inproceedings{zhang2021lorentzian,
  title={Lorentzian graph convolutional networks},
  author={Zhang, Yiding and Wang, Xiao and Shi, Chuan and Liu, Nian and Song, Guojie},
  booktitle={Proceedings of the Web Conference 2021},
  pages={1249--1261},
  year={2021}
}

@inproceedings{tabaghi2020hyperbolic,
  title={Hyperbolic distance matrices},
  author={Tabaghi, Puoya and Dokmani{\'c}, Ivan},
  booktitle={Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={1728--1738},
  year={2020}
}

@inproceedings{cai2023cyclic,
  title={Cyclic block coordinate descent with variance reduction for composite nonconvex optimization},
  author={Cai, Xufeng and Song, Chaobing and Wright, Stephen and Diakonikolas, Jelena},
  booktitle={International Conference on Machine Learning},
  pages={3469--3494},
  year={2023},
  organization={PMLR}
}

@article{schmidt2017minimizing,
  title={Minimizing finite sums with the stochastic average gradient},
  author={Schmidt, Mark and Le Roux, Nicolas and Bach, Francis},
  journal={Mathematical Programming},
  volume={162},
  pages={83--112},
  year={2017},
  publisher={Springer}
}

@inproceedings{li2021page,
  title={PAGE: A simple and optimal probabilistic gradient estimator for nonconvex optimization},
  author={Li, Zhize and Bao, Hongyan and Zhang, Xiangliang and Richt{\'a}rik, Peter},
  booktitle={International conference on machine learning},
  pages={6286--6295},
  year={2021},
  organization={PMLR}
}

@article{cutkosky2019momentum,
  title={Momentum-based variance reduction in non-convex sgd},
  author={Cutkosky, Ashok and Orabona, Francesco},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}
@article{HeY12,
  author    = {Bingsheng He and
               Xiaoming Yuan},
  title     = {On the $\mathcal{O}(1/n)$ Convergence Rate of the Douglas-Rachford Alternating
               Direction Method},
  journal   = {SIAM Journal on Numerical Analysis },
  volume    = {50},
  number    = {2},
  year      = {2012},
  pages     = {700-709},
}

@article{attouch2010proximal,
  title={Proximal alternating minimization and projection methods for nonconvex problems: An approach based on the Kurdyka-{\L}ojasiewicz inequality},
  author={Attouch, H{\'e}dy and Bolte, J{\'e}r{\^o}me and Redont, Patrick and Soubeyran, Antoine},
  journal={Mathematics of operations research},
  volume={35},
  number={2},
  pages={438--457},
  year={2010},
  publisher={INFORMS}
}
@article{defazio2014saga,
  title={SAGA: A fast incremental gradient method with support for non-strongly convex composite objectives},
  author={Defazio, Aaron and Bach, Francis and Lacoste-Julien, Simon},
  journal={Advances in neural information processing systems},
  volume={27},
  year={2014}
}
@inproceedings{NIPS2013TongZ,
 author = {Johnson, Rie and Zhang, Tong},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {C.J. Burges and L. Bottou and M. Welling and Z. Ghahramani and K.Q. Weinberger},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Accelerating Stochastic Gradient Descent using Predictive Variance Reduction},
 volume = {26},
 year = {2013}
}
@inproceedings{nguyen2017sarah,
  title={SARAH: A novel method for machine learning problems using stochastic recursive gradient},
  author={Nguyen, Lam M and Liu, Jie and Scheinberg, Katya and Tak\'a\v{c}, Martin},
  booktitle={International conference on machine learning},
  pages={2613--2621},
  year={2017},
  organization={PMLR}
}
@article{zhou2020stochastic,
  title={Stochastic nested variance reduction for nonconvex optimization},
  author={Zhou, Dongruo and Xu, Pan and Gu, Quanquan},
  journal={The Journal of Machine Learning Research},
  volume={21},
  number={1},
  pages={4130--4192},
  year={2020},
  publisher={JMLRORG}
}
@article{fang2018spider,
  title={Spider: Near-optimal non-convex optimization via stochastic path-integrated differential estimator},
  author={Fang, Cong and Li, Chris Junchi and Lin, Zhouchen and Zhang, Tong},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@article{wang2019spiderboost,
  title={Spiderboost and momentum: Faster variance reduction algorithms},
  author={Wang, Zhe and Ji, Kaiyi and Zhou, Yi and Liang, Yingbin and Tarokh, Vahid},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@inproceedings{li2017convergence,
  title={Convergence analysis of proximal gradient with momentum for nonconvex optimization},
  author={Li, Qunwei and Zhou, Yi and Liang, Yingbin and Varshney, Pramod K},
  booktitle={International Conference on Machine Learning},
  pages={2111--2119},
  year={2017},
  organization={PMLR}
}
@article{j2016proximal,
  title={Proximal stochastic methods for nonsmooth nonconvex finite-sum optimization},
  author={J Reddi, Sashank and Sra, Suvrit and Poczos, Barnabas and Smola, Alexander J},
  journal={Advances in neural information processing systems},
  volume={29},
  year={2016}
}


@article{ghadimi2016mini,
  title={Mini-batch stochastic approximation methods for nonconvex stochastic composite optimization},
  author={Ghadimi, Saeed and Lan, Guanghui and Zhang, Hongchao},
  journal={Mathematical Programming},
  volume={155},
  number={1-2},
  pages={267--305},
  year={2016},
  publisher={Springer}
}
@inproceedings{NEURIPS2018,
 author = {Fang, Cong and Li, Chris Junchi and Lin, Zhouchen and Zhang, Tong},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Bengio and H. Wallach and H. Larochelle and K. Grauman and N. Cesa-Bianchi and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {SPIDER: Near-Optimal Non-Convex Optimization via Stochastic Path-Integrated Differential Estimator},
 volume = {31},
 year = {2018}
}

@book{absil2008optimization,
  title={Optimization algorithms on matrix manifolds},
  author={Absil, P-A and Mahony, Robert and Sepulchre, Rodolphe},
  year={2008},
  publisher={Princeton University Press}
}

@book{golub2013matrix,
  title={Matrix computations},
  author={Golub, Gene H and Van Loan, Charles F},
  year={2013},
  publisher={JHU press}
}

@article{gao2019parallelizable,
  title={Parallelizable algorithms for optimization problems with orthogonality constraints},
  author={Gao, Bin and Liu, Xin and Yuan, Ya-xiang},
  journal={SIAM Journal on Scientific Computing},
  volume={41},
  number={3},
  pages={A1949--A1983},
  year={2019},
  publisher={SIAM}
}

@article{vsego2010two,
  title={Two-sided hyperbolic SVD},
  author={{\v{S}}ego, Vedran},
  journal={Linear algebra and its applications},
  volume={433},
  number={7},
  pages={1265--1275},
  year={2010},
  publisher={Elsevier}
}

@article{novakovic2022kogbetliantz,
  title={A Kogbetliantz-type algorithm for the hyperbolic SVD},
  author={Novakovi{\'c}, Vedran and Singer, Sanja},
  journal={Numerical algorithms},
  volume={90},
  number={2},
  pages={523--561},
  year={2022},
  publisher={Springer}
}

@inproceedings{hui2022low,
  title={Low-rank nonnegative tensor decomposition in hyperbolic space},
  author={Hui, Bo and Ku, Wei-Shinn},
  booktitle={Proceedings of the 28th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={646--654},
  year={2022}
}

@inproceedings{zeng2019global,
  title={Global convergence of block coordinate descent in deep learning},
  author={Zeng, Jinshan and Lau, Tim Tsz-Kit and Lin, Shaobo and Yao, Yuan},
  booktitle={International conference on machine learning},
  pages={7313--7323},
  year={2019},
  organization={PMLR}
}

@inproceedings{huang2021riemannian,
  title={A riemannian block coordinate descent method for computing the projection robust wasserstein distance},
  author={Huang, Minhui and Ma, Shiqian and Lai, Lifeng},
  booktitle={International Conference on Machine Learning},
  pages={4446--4455},
  year={2021},
  organization={PMLR}
}

@inproceedings{wu2021federated,
  title={Federated block coordinate descent scheme for learning global and personalized models},
  author={Wu, Ruiyuan and Scaglione, Anna and Wai, Hoi-To and Karakoc, Nurullah and Hreinsson, Kari and Ma, Wing-Kin},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={12},
  pages={10355--10362},
  year={2021}
}

@inproceedings{cai2021zeroth,
  title={A zeroth-order block coordinate descent algorithm for huge-scale black-box optimization},
  author={Cai, HanQin and Lou, Yuchen and McKenzie, Daniel and Yin, Wotao},
  booktitle={International Conference on Machine Learning},
  pages={1193--1203},
  year={2021},
  organization={PMLR}
}

@article{nutini2022let,
  title={Let's make block coordinate descent converge faster: faster greedy rules, message-passing, active-set complexity, and superlinear convergence},
  author={Nutini, Julie and Laradji, Issam and Schmidt, Mark},
  journal={Journal of Machine Learning Research},
  volume={23},
  number={131},
  pages={1--74},
  year={2022}
}

@inproceedings{yuan2023coordinate,
  title={Coordinate descent methods for dc minimization: Optimality conditions and global convergence},
  author={Yuan, Ganzhao},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={37},
  number={9},
  pages={11034--11042},
  year={2023}
}

@article{yang2024practical,
  title={A Practical Beamforming Design for Active RIS-assisted MU-MISO Systems},
  author={Yang, Yun and Lu, Zhiping and Li, Ming and Liu, Rang and Liu, Qian},
  journal={arXiv preprint arXiv:2401.03873},
  year={2024}
}

@inproceedings{ma2020hsic,
  title={The HSIC bottleneck: Deep learning without back-propagation},
  author={Ma, Wan-Duo Kurt and Lewis, JP and Kleijn, W Bastiaan},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={34},
  number={04},
  pages={5085--5092},
  year={2020}
}

@article{sabne2017model,
  title={Model-based iterative CT image reconstruction on GPUs},
  author={Sabne, Amit and Wang, Xiao and Kisner, Sherman J and Bouman, Charles A and Raghunathan, Anand and Midkiff, Samuel P},
  journal={ACM SIGPLAN Notices},
  volume={52},
  number={8},
  pages={207--220},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@article{law2020ultrahyperbolic,
  title={Ultrahyperbolic representation learning},
  author={Law, Marc and Stam, Jos},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1668--1678},
  year={2020}
}

@article{hansen1963cyclic,
  title={On cyclic Jacobi methods},
  author={Hansen, Eldon R},
  journal={Journal of the Society for Industrial and Applied Mathematics},
  volume={11},
  number={2},
  pages={448--459},
  year={1963},
  publisher={SIAM}
}

@article{hari2021convergence,
  title={On the convergence of complex Jacobi methods},
  author={Hari, Vjeran and Kova{\v{c}}, Erna Begovi{\'c}},
  journal={Linear and multilinear algebra},
  volume={69},
  number={3},
  pages={489--514},
  year={2021},
  publisher={Taylor \& Francis}
}
